Adaptive Masking Enhances Visual Grounding

In recent years, zero-shot and few-shot learning in visual grounding have garnered considerable attention, largely due to the success of large-scale vision-language pre-training on expansive datasets such as LAION-5B and DataComp-1B. However, the continuous expansion of these datasets presents significant challenges, particularly with respect to data availability and computational overhead, thus creating a bottleneck in the advancement of low-shot learning capabilities. In this paper, we propose IMAGE, Interpretative MAsking with Gaussian radiation modEling, aimed at enhancing vocabulary grounding in low-shot learning scenarios without necessitating an increase in dataset size. Drawing inspiration from cognitive science and the recent success of masked autoencoders (MAE), our method leverages adaptive masking on salient regions of the feature maps generated by the vision backbone. This enables the model to learn robust, generalized representations through the reconstruction of occluded information, thereby facilitating effective attention to both local and global features. We evaluate the efficacy of our approach on benchmark datasets, including COCO and ODinW, demonstrating its superior performance in zero-shot and few-shot tasks. Experimental results consistently show that IMAGE outperforms baseline models, achieving enhanced generalization and improved performance in low-shot scenarios. These findings highlight the potential of adaptive feature manipulation through attention mechanisms and Gaussian modeling as a promising alternative to approaches that rely on the continual scaling of dataset sizes for the advancement of zero-shot and few-shot learning. Our code is publicly available at https://github.com/git-lenny/IMAGE.

==> secs/3_method_bak2.tex <==
\section{Method}

\begin{figure*}[ht]
   \centering
   \includegraphics[width=\linewidth]{figs/pipeline_3.pdf} 
   \caption{Pipeline of IMAGE model, consisting of two blocks: attention prior generation module and RF-GAM mask generation module.}
   \label{fig:scaling_laws}
\end{figure*}

\textbf{IMAGE} aims to enhance zero-shot and few-shot visual grounding without relying on large-scale datasets. Inspired by Masked Autoencoders (MAE), IMAGE leverages adaptive masking techniques that emphasize salient regions within an image's feature map, compelling the model to infer missing information and learn robust, generalized representations. As is shown in fig(???) IMAGE consists of two primary components: the \textbf{Importance Prior Generation Block} ($\theta_p$), which estimates the importance of image patches based on their relationships within the feature map, and the \textbf{Adaptive Mask Generation Block} ($\theta_m$), which creates adaptive masks guided by the importance prior to direct the model’s attention during training. Given an input image, a pretrained Swin-Transformer backbone network processes it to produce hierarchical feature maps at multiple scales, denoted as $\{F_1, F_2, F_3, F_4\}$, where each feature map $F_i$ has dimensions $(B, C_i, H_i, W_i)$, representing batch size $B$, number of channels $C_i$, and spatial dimensions $H_i \times W_i$ at scale $i$. IMAGE applies adaptive masking on these feature maps, focusing the model's attention on the most relevant regions, thereby improving its reasoning capabilities and generalization performance.

\subsection{Importance Prior Generation}

The first step in adaptive masking is to compute an \textit{importance prior} that captures the relevance of each patch within a feature map. For each feature map $F_i$, we perform the following steps:

\paragraph{Self-Attention Encoding}

We reshape $F_i$ into a sequence of tokens and apply a self-attention mechanism to capture contextual relationships between image patches:
\begin{align*}
X_i &= \text{Reshape}(F_i) \in \mathbb{R}^{B \times N_i \times C_i}, \\ 
Z_i &= X_i + \text{SelfAttention}(X_i), \\
T_i &= Z_i + \text{FFN}(Z_i),
\end{align*}
where $N_i = H_i \times W_i$ is the number of patches at scale $i$, and $\text{FFN}$ denotes a feedforward network.

\paragraph{Importance Calculation}

To compute the importance of each patch, we calculate the correlation between each patch $p_j$ and all other patches in $T_i$:
\[
S_j = p_j \times T_i^\top,
\]
where $p_j \in \mathbb{R}^{B \times 1 \times C_i}$ is the feature vector of the $j$-th patch. We then average $S_j$ over all patches to obtain the importance score for patch $p_j$:
\[
s_j = \text{AveragePooling}(S_j).
\]
Repeating this for all patches yields the importance prior matrix $S_{\text{whole}} \in \mathbb{R}^{B \times N_i \times 1}$. We normalize the importance scores to ensure comparability:
\[
\widetilde{S}_{\text{whole}} = \frac{S_{\text{whole}} - \min(S_{\text{whole}})}{\max(S_{\text{whole}}) - \min(S_{\text{whole}})}.
\]

\subsection{Adaptive Mask Generation}

Using the importance prior $\widetilde{S}_{\text{whole}}$, we generate adaptive masks that obscure certain patches based on their importance. We propose two methods:

\paragraph{Threshold-Based Adaptive Masking} We sort the patches based on their importance scores and designate the top $\rho_i\%$ as important regions for each scale $i$. Within these important regions, we randomly select $\gamma\%$ of the patches to apply masking. For the remaining patches, we randomly mask patches to meet the desired masking ratio $\rho_i$. This strategy challenges the model to infer critical information from incomplete data while ensuring it has sufficient information to learn effectively.

\paragraph{Radiance Field Gaussian Adaptive Masking (RF-GAM)}

To implement a spatially aware masking strategy, we model the importance distribution using Gaussian radiance fields. For each feature map $F_i$, we select the top $K_i$ patches as radiation points based on their importance scores. For each radiation point $k$, we estimate its variance $\sigma_k^2$ by combining its feature vector $f_k$ with the cross-attention output $c_k$ and passing it through a feedforward network:

\begin{align*}
h_k &= [f_k, c_k], \\
\sigma_k^2 &= \text{ReLU}(\text{FFN}_\sigma(h_k)) + \epsilon,
\end{align*}

where $\epsilon$ ensures numerical stability. The radiance intensity at each location $(x, y)$ is computed as:

\[
I^{(b)}(x,y) = \sum_{k=1}^{K_i} \alpha_k^{(b)} \exp\left( -\frac{\| (x,y) - (x_k, y_k) \|^2}{2\sigma_k^{2(b)}} \right),
\]

where $\alpha_k^{(b)}$ is the amplitude (importance score) of radiation point $k$. We determine masking thresholds based on the intensity distribution's mean $\mu^{(b)}$ and standard deviation $\sigma^{(b)}$:

\begin{align*}
T_{\text{hard}}^{(b)} &= \mu^{(b)} + (\delta + k)\sigma^{(b)}, \\
T_{\text{no-mask}}^{(b)} &= \mu^{(b)} + (\delta - k)\sigma^{(b)},
\end{align*}

with hyperparameters $\delta$ and $k$. The mask $M_i^{(b,p)}$ is defined as:

\[
M_i^{(b,p)} = 
\begin{cases}
0, & \text{if } I^{(b)}(x,y) > T_{\text{hard}}^{(b)}, \\
1, & \text{if } I^{(b)}(x,y) < T_{\text{no-mask}}^{(b)}, \\
1 - \dfrac{I^{(b)}(x,y) - T_{\text{no-mask}}^{(b)}}{T_{\text{hard}}^{(b)} - T_{\text{no-mask}}^{(b)}}, & \text{otherwise}.
\end{cases}
\]

The final mask $M_i \in [0,1]^{B \times N_i}$ is applied to the feature map:

\[
F_i^{\prime} = F_i \odot \text{Reshape}(M_i),
\]

where $\odot$ denotes element-wise multiplication.


\paragraph{Progressive Masking Strategy}

To ensure effective learning, we introduce a progressive masking strategy that adjusts the masking ratio over the course of training:

\begin{itemize}
    \item \textbf{Multi-Scale Masking}: Apply different masking ratios at different feature map scales. Lower-level feature maps retain more detail, while higher-level maps have higher masking ratios to focus on reasoning.
    \item \textbf{Dynamic Masking}: Gradually increase the masking ratio and mask strength during training. The hyperparameter $k$ in RF-GAM is adjusted per epoch:
    \[
    k_{\text{epoch}} = k_0 \left(1 - \frac{\text{epoch}}{E_{\text{total}}}\right),
    \]
    where $k_0$ is the initial value, and $E_{\text{total}}$ is the total number of training epochs.
\end{itemize}

This progressive approach allows the model to adapt to increasing levels of difficulty, enhancing its ability to infer missing information and learn robust representations.

\subsection{Theoretical Analysis}

We provide a theoretical justification for how adaptive masking improves performance, drawing parallels to the principles of generalization.

\begin{assumption}
The IAMGE model is trained on a dataset of image-text pairs $(x_i, t_i)$ drawn i.i.d. from an unknown joint distribution $\mathcal{D}$. Each image $x_i$ is encoded into a feature map $\mathcal{F}_i$, and the adaptive masking function generates a mask matrix $\mathcal{M}_i$ based on the importance prior learned from the feature map.
\end{assumption}

\begin{assumption}
The masking loss $L_{\text{mask}}$ is $L$-Lipschitz continuous with respect to the masked feature map $\mathcal{F}_i^{\prime} = \mathcal{F}_i \odot \mathcal{M}_i$, where $\odot$ denotes element-wise multiplication.
\end{assumption}

\begin{lemma}
Let $\hat{y}_{ij}$ be the predicted similarity between the masked image feature embedding and the corresponding text embedding in a batch. Let $y^*_{ij}$ be the optimal similarity that minimizes the IMAGE loss $L_{\text{IMAGE}}$. Then, with probability at least $1-\delta$, we have:
\[
|\hat{y}_{ij} - y^*_{ij}| \leq \frac{1}{\tau} \sqrt{\frac{\log(2/\delta)}{2N_{\text{batch}}}} + \frac{\beta L}{\tau},
\]
where $\tau$ is the temperature hyperparameter, $\beta$ is the masking loss weight, and $N_{\text{batch}}$ is the batch size.
\end{lemma}

\begin{proof}
The first term arises from Hoeffding's inequality, which bounds the deviation between the empirical mean $\hat{y}_{ij}$ and the true expectation $y^*_{ij}$ of the similarity between masked image features and text embeddings. Since $0 \leq \hat{y}_{ij} \leq 1$, the deviation is bounded by:
\[
\mathbb{P}\left(|\hat{y}_{ij} - \mathbb{E}[\hat{y}_{ij}]| \geq \epsilon\right) \leq 2 \exp\left(-2N_{\text{batch}}\epsilon^2\right).
\]
Solving for $\epsilon$ with probability $1 - \delta$ gives the first term.

The second term follows from the Lipschitz continuity of $L_{\text{mask}}$. By Assumption 2, for any two masked feature maps $\mathcal{F}_i^{\prime}$ and $\mathcal{F}_i^{\prime\prime}$, we have:
\[
|L_{\text{mask}}(\mathcal{F}_i^{\prime}) - L_{\text{mask}}(\mathcal{F}_i^{\prime\prime})| \leq L \|\mathcal{F}_i^{\prime} - \mathcal{F}_i^{\prime\prime}\|.
\]
The deviation between the masked features of $\hat{y}$ and $y^*$ is bounded by their total variation distance, scaled by the Lipschitz constant and the loss weight $\beta$. Combining both terms completes the proof.
\end{proof}

\begin{theorem}[\textbf{IMAGE Generalization Bound}]
Let $f_\theta$ denote the IMAGE model with learned parameters $\theta$. Let $\hat{R}(f_\theta)$ and $R(f_\theta)$ denote its empirical and expected risks, respectively, on a downstream task. Then, with probability at least $1 - \delta$ over the training set, we have:
\[
R(f_\theta) \leq \hat{R}(f_\theta) + \mathcal{O}\left(\frac{1}{\tau}\sqrt{\frac{\log(1/\delta)}{N_{\text{batch}}}} + \frac{\beta L}{\tau}\right).
\]
\end{theorem}

\begin{proof}
The empirical risk $\hat{R}(f_\theta)$ is an average over the predicted similarities $\hat{y}_{ij}$ for image-text pairs in the masked feature space. By Lemma 1 and applying a union bound over all $O(N_{\text{batch}}^2)$ pairs, each term $\hat{y}_{ij}$ concentrates around the optimal $y^*_{ij}$ with high probability. The total deviation is bounded by:
\[
|\hat{R}(f_\theta) - R(f_\theta)| \leq \frac{1}{\tau} \sqrt{\frac{\log(2N_{\text{batch}}^2/\delta)}{2N_{\text{batch}}}} + \frac{\beta L}{\tau}.
\]
Simplifying the logarithmic term and constants yields the stated bound.
\end{proof}

\paragraph{Discussion.}

The theoretical analysis demonstrates that adaptive masking contributes to reducing the generalization error by forcing the model to learn robust representations from incomplete data. The generalization bound indicates that the error decreases with larger batch sizes $N_{\text{batch}}$ and appropriate choices of the temperature parameter $\tau$, masking loss weight $\beta$, and Lipschitz constant $L$. By adaptively masking key regions, the model is encouraged to develop stronger reasoning capabilities, which translates to improved performance in zero-shot and few-shot tasks.

\subsection{Optimization and Learning Strategy}

To optimize the model effectively, we employ the following learning strategies:

\begin{itemize}
    \item \textbf{Loss Functions}: We combine the standard contrastive loss used in vision-language pre-training with the masking loss $L_{\text{mask}}$, weighted by $\beta$:
    \[
    L_{\text{total}} = L_{\text{contrastive}} + \beta L_{\text{mask}}.
    \]
    \item \textbf{Training Schedule}: We adopt an asymptotic learning schedule, gradually increasing the masking difficulty as the model becomes more capable.
    \item \textbf{Hyperparameter Tuning}: Parameters such as the initial masking ratio, the rate of increase, and the thresholds in RF-GAM are tuned to balance the trade-off between learning from sufficient information and challenging the model.
\end{itemize}

By integrating the adaptive masking technique with a carefully designed optimization strategy, IMAGE effectively enhances the model's ability to generalize from limited data without the need for scaling up dataset size.


==> secs/3_method_old.tex <==
\section{Method}

\begin{figure}[t!]
  \includegraphics[width=\linewidth]{figs/pipeline2.pdf}
  \caption{Pipeline of the model.}
  \label{fig:pipeline}
\end{figure}
 The primary objective of our method is to address the inherent challenges of low-shot grounding by leveraging adaptive masking techniques that dynamically focus on salient features within an image. Specifically, given a feature map $\mathcal{F} \in \mathbb{R}^{C\times H\times W}$, the goal of the adaptive masking module is to generate the corresponding mask matrix  $\mathcal{M} \in \mathbb{R}^{1\times H\times W}$ to mask the key features in the feature map. By employing a mask $M$ that selectively highlights important regions in the image feature $F$, we aim to teach the model to pay more attention on the object's important features and reason them.

We propose AMAZE, $\theta_{amaze}$, for boosting model's low-shot grounding capabilities without utilizing larger datasets, which consists of an importance prior generation block $\theta_{p}$ and an adaptive mask generation block $\theta_{m}$. First, we utilize $\theta_{p}$ to obtain an importance prior based on the feature map. The mask $M$ is then computed based on the learned importance of different patches regions. The core idea of AMAZE is to utilize the two blocks for applying adaptive masks to the feature maps encoded by the image encoder, strategically obscuring important regions to challenge the model during training. By forcing the model to infer key missing information, we encourage it to develop more robust representations that generalize better to new, unseen data. 


% \subsection{Preliminary Knowledge of Autoregressive Modeling}
\subsection{Importance Prior Modeling}
The first step in our adaptive mask module is to model the importance of image patches extracted from the backbone network. By quantifying the significance of each patch, we can guide the subsequent mask generation process to focus on critical regions of the image, enhancing the model's ability to learn robust representations and reason on the image feature.

Specially, we utilize a pretrained Swin-Transformer as our framework's image encoder, which processes the input image and outputs a set of hierarchical feature maps at multiple scales:
\begin{align}
\{F_1, F_2, F_3, F_4\},
\end{align}
Each feature map $F_i$ has dimensions $(B, C_i, H_i, W_i)$, where B is the batch size, $C_i$ is the number of channels, and $H_i \times W_i$ are the spatial dimensions at scale i.

Given the feature map $F_i$, To capture the relationships between patches, we first encode the feature maps using a residual self-attention module followed by a feedforward network, whcih strengthen the relationships between patches. We reshape the $F_i$ into a sequence of tokens, then we apply a self-attention mechanism to capture the contextual relationships and the output of the self-attention layer is passed through an FFN to enhance the feature representations.
\begin{align*}
X_i &= Reshape(F_i) \in \mathbb{R}^{B \times N_i \times C_i}, \\ Z_i &= X_i + SelfAttention(X_i), \\
T_i &= Z_i + FFN(Z_i)
\end{align*}
For calculating the importance of each patch, we use a simple yet effective method. We get the importance map by calculating the correlation importance between patches with average pooling. Given a patch $p_j \in \mathbb{R}^{B \times 1 \times C_i}$ selected from $T_i \in \mathbb{R}^{B \times N_i \times C_i}$ at the $j^\text{th}$ position, The correlation importance between $p_j$ and all $N$ patches can be computed as:
\begin{align}
S_j = p_j \times T_i^T,
\end{align}
Where $S_j \in \mathbb{R}^{B \times N_i}$. Then, we conduct average pooling on $S_j$ to obtain the importance ${S^{'}_j} \in \mathbb{R}^{B \times 1}$ of $p_j$ on the feature map. By performing this operation to all $N_i$ patches on the feature map, we can get the whole correlation importance map, which can be expressed as:
\begin{align*}
S_{\text{whole}} = AveragePooling(T_i \times T_i^T),
\end{align*}
Where $S_\text{whole} \in \mathbb{R}^{B \times B_i \times 1}$. In the end, we normalize the importance scores across patches to ensure they are comparable:
\begin{align*}
\widetilde{S}_{\text{whole}} = \frac{S_k - min(S_\text{whole})}{max(S_\text{whole}) - min(S_\text{whole})},
\end{align*}
In this way, We subtly design an adapter and utilize the attention weight matrix to model the importance prior on the feature map.

\subsection{Adaptive Mask Generation}
Given the importance prior map, we generate adaptive masks that strategically mask or obscure certain patches to guide the model focusing on important patches' features and boosting its reasoning ablility. We propose two methods for adaptive masks generation: $(1)$ Threshold-Based Adaptive Masking, and $(2)$ Radiance Field Gaussian Adaptive Masking (RF-GAM).

For threshold-based adaptive masking, given each feature map $F_i$ and importance prior matrix $\widetilde{S}_{\text{whole}}$, we flattened the patches from the feature map and sort them based on $\widetilde{S}_{\text{whole}}$. Specially, we designate the top $\rho_i\%$ of the patches as important regions, where $\rho_i$ is a predefined hyperparameter for each scale (e.g., $30\%$ for the first scale, $40\%$ for the second, etc.). Within the important regions, we randomly select $\gamma\%$ of the patches to apply masking. This challenges the model to infer critical information from incomplete data, while avoiding that all information is obscured to the extent that the model can not learn. In the remaining patches, we randomly mask patches to ensure the total number of masked patches meets the desired masking ratio $\rho_i$ for scale $i$.


An important point of RF-GAM is that spatially proximate patches of an image tend to be more strongly correlated(???). As a result, to introduce a more flexible and spatially aware masking strategy, we model the importance distribution using Gaussian radiance fields. For each feature map $F_i$ and its corresponding importance prior matrix $\widetilde{S}_{\text{whole}}$, we select the top $K_i$ patches based on their importance scores in importance prior matrix and treat them as radiation points. In order to determine the location, variance and amplitude of the radiation point $k$, intuitively, we consider the corresponding normalized spatial coordinates $(x_k, y_k)$ in the feature map and importance scores $\alpha_k = {\widetilde{s_i}^{(b,p_k)}}$ in importance prior matrix as the center coordinates and amplitude of the field, respectively. To acquire accurate variance for each radiation point, we conduct variance estimation process through a cross-attention and feed forward module. Concretely, we treat the feature vector of the radiation point $f_k = T_i^{(b,p_k)} \in \mathbb{R}^{C_i}$ and all patch features in $T_i$, $f_j = \{T^{(b,j)}\}_{j=1}^{N_i}$ as query and key, values respectively. Then we get the radiation feature enhanced features denoted as $c_k = CrossAttention(f_k, f_j, f_j)$. In the end, the accurate variance obtained by concatenating the query and the features, and passing through an FFN module:
\begin{align*}
h_k &= [f_k, c_k], \\
\sigma_k^2 &= RELU(FFN_\sigma(h_k)) + \epsilon,
\end{align*}
where $\epsilon$ is a small constant to ensure numerical stability, and $RELU$ ensures the variance is non-negative. Given the spatial coordinates $(x_k, y_k)$, amplitude $\alpha_k$ and variance $\sigma$, The radiance intensity $I^(b)(x,y)$ at each spatial location $(x,y)$ can be computed as:
\begin{align}
I^{(b)}(x,y) = \sum^{K_i}_{k=1}\alpha_k^{(b)}exp{(-\frac{\parallel(x,y) - (x_k,y_k)\parallel^2}{2\sigma_k^{2(b)}})}, 
\end{align}

It can be shown that the intensity distribution of this intensity matrix also obeys a Gaussian distribution and easy to compute its mean $\mu^{(b)}$ and variance $\sigma^{(b)}$. We set two threshold for hard masking and soft masking respectively based on $\mu^{(b)}$ and $\sigma^{(b)}$ , which makes us adopt hard masks and soft masks on different feature regions flexibly:
\begin{align}
T_\text{hard}^{(b)} = \mu^{(b)} + (\delta + k)\sigma^{(b)}, \\
T_\text{no\_mask}^{(b)} = \mu^{(b)} + (\delta - k)\sigma^{(b)}, 
\end{align}

Where $\delta$ and $k$ are the hyperparameters in network. Based on $T_\text{hard}^{(b)}$ and $T_\text{no\_mask}^{(b)}$, we conduct hard masking scheme and no masking on patches with $I^{(b)}(x,y) > T_\text{hard}^{(b)}$ and $I^{(b)}(x,y) < T_\text{no\_mask}^{(b)}$ respectively. For patches in between, we subtly design an adaptive method for soft masking intensity, which can be summarized as the higher the intensity of the patches, the stronger the soft masks:
\begin{align}
M_i^{(b,p)} = 1 - \frac{I^{(b)}(x,y) - T_\text{no\_mask}^{(b)}}{T_\text{hard}^{(b)} - T_\text{no\_mask}^{(b)}}
\end{align}

 By both, we adaptively create a binary mask $M_i \in {\{0,1\}}^{B \times N_i}$ for each feature map, where $M_i^{(b,p)} = 0$ if patch $p$ in batch $b$ is to be masked, while $M_i^{(b,p)} = 1$ otherwise. The masked feature map $F^{'}_i$ is obtained by: $F^{'}_i = F_i \odot Reshape(M_i)$, where $\odot$ denotes element-wise multiplication and $M_i$ is reshaped to match the dimension of $F_i$.


\subsection{Optimization for Learning Strategy}
We craft the progressive learning strategy in terms of multiple scales and training processes to ensure that the model can adapt itself and adjust to the gradual masking process. At the multi-scale point, we impose different masking ratios on different feature maps, while gradually increasing the masking ratio on each layer of feature maps during the training process.

Specially, given the feature maps from the image encoder, we would like to keep some details on the bottom-level feature maps so that the model does not fail to learn because it can not access to enough features. At the high level feature maps, however, we will mask out a significant percentage of the patches to force the model performing inference on the important reasons and learn robust representations. In this way, the model can reason and learn the representation as much as possible in the absence of information, while retaining the necessary information for the learning process.

On the other hand, to avoid the model to perform too difficult inference in the early stage of training, we adopt an asymptotically learning ground dynamic masking strategy, i.e., during the early stage of training, we apply a few number of lighter masks on the feature maps, and as the number of training epochs increases, we gradually increase the number of masks and the strength of the masks in the important regions. In RF-GAM, as the $T_\text{hard}^{(b)}$ and $T_\text{no\_mask}^{(b)}$ can be determined by $\mu$, $\sigma$, $\delta$ and $k$, where $\mu$, $\sigma$ and $\delta$ are the determined value, we set hyperparameter $k$ as: $k_\text{epoch} = k_0 \dot (1 - \frac{epcoh}{E_\text{total}})$. It is clear that k is decreasing with the number of training epochs, allowing for the translation of the sigma window and dynamically increasing the number of hard masks. In this way, we can learn asymptotically in a probability window based manner during training.

By controlling the proportion of hard masks at multiple levels of the feature map and training process, we achieve fruitful learning optimization and function convergence.



==> secs/tem.tex <==



Controllable generation is a critical and widely applicable area in the field of generative models, which has recently seen significant progress. Diffusion models~\citep{song2020denoising, ho2020denoising}, which are based on iteratively denoising noise using a Markov chain, have demonstrated impressive generation capabilities and have given rise to a series of excellent controllable generation methods, such as ControlNet~\citep{zhang2023adding} and T2I Adapter~\citep{mou2024t2i}. These methods allow fine-grained control through additional signals like edge maps and human poses. However, diffusion models face two main challenges: 1) the iterative diffusion steps result in high computational costs, and 2) their representations are inconsistent with popular large language models (LLMs)~\citep{chiang2023vicuna, touvron2023llama}, hindering seamless integration in multimodal tasks. These limitations highlight the need for more efficient and unified controllable generative paradigms.

Inspired by recent autoregressive language modeling~\citep{radford2019language, brown2020language}, autoregressive visual modeling has been explored as a scalable alternative due to its potential to address the shortcomings of diffusion models. Through careful design, works such as VQ-VAE~\citep{van2017neural}, DALL-E~\citep{ramesh2021zero}, and VAR~\citep{tian2024visual} demonstrate generative capabilities comparable to those of diffusion models. However, current autoregressive paradigms have not deeply explored controllable generation. Some recent works, such as IQ-VAE~\citep{zhan2022auto}, use condition patches as prefix tokens to generate subsequent image patches, resulting in overly long sequence modeling. ControlVAR~
\citep{li2024controlvar}, by contrast, models both conditions and images simultaneously but limits the ability to leverage pre-trained models and lacks flexibility. Overall, current autoregressive approaches in controllable generation exhibit inefficiencies and limited controllability. To address these challenges, we aim to propose a flexible, efficient, and plug-and-play controllable framework based on pre-trained autoregressive models.

In this paper, we propose CAR, an end-to-end, plug-and-play model that learns conditional control for a pre-trained visual autoregressive model. By freezing the weights of the pre-trained model, we preserve its generative capability, ensuring high final image quality while reducing training overhead. We refer to the control branch as the Conditional Autoregressive Model, which runs in parallel with the pre-trained model. Features from the conditional image are extracted at different scales and serve as input tokens for the Conditional Autoregressive Model. Autoregressive modeling is applied to these tokens, with each scale attending only to its prefix scales, enabling the learning of multi-scale conditional control information. This conditional information is injected into the pre-trained autoregressive model via normalized injection.
